Ranking Policy Gradient

Sample inefficiency is a long-lasting problem in reinforcement learning (RL). The state-of-the-art estimates the optimal action values while it usually involves an extensive search over the state-action space and unstable optimization. Towards the sample-efficient RL, we propose ranking policy gradient (RPG), a policy gradient method that learns the optimal rank of a set of discrete actions. To accelerate the learning of policy gradient methods, we establish the equivalence between maximizing the lower bound of return and imitating a near-optimal policy without accessing any oracles. These results lead to a general off-policy learning framework, which preserves the optimality, reduces variance, and improves the sample-efficiency. Furthermore, the sample complexity of RPG does not depend on the dimension of state space, which enables RPG for large-scale problems. We conduct extensive experiments showing that when consolidating with the off-policy learning framework, RPG substantially reduces the sample complexity, comparing to the state-of-the-art.

==> bmacros.tex <==
%% common packages
\usepackage{amsbsy}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{color}
\usepackage{booktabs}

%% to allow citation as footnote
\usepackage{natbib}
% and to reduce footnote font size
\usepackage{etoolbox}
\makeatletter
\patchcmd{\@makefntext}{\insertfootnotetext{#1}}{\insertfootnotetext{\scriptsize#1}}{}{}
\makeatother


%% macros for commenting
\usepackage[normalem]{ulem} % to use \sout
\newcommand{\remove}[1]{{\color{Gray}\sout{#1}}}
\newcommand{\revise}[1]{{\color{blue}#1}}
\newcommand{\commwy}[1]{{\color{red}(wy: #1)}} % Wotao Yin

%% template for beamer

%\mode<presentation>
%{
%  % page number
%  %\setbeamertemplate{footline}{\insertframenumber/\inserttotalframenumber}
%  \setbeamertemplate{footline}[frame number]
%
%  % background and theme
%  \setbeamertemplate{background canvas}[vertical shading][bottom=white!10,top=white!10]
%  \usetheme{default}
%
%  % section in table of contents has numbers
%  \setbeamertemplate{sections/subsections in toc}[sections numbered]
%
%  % no navigation bottoms
%  \setbeamertemplate{navigation symbols}{}
%
%  % itemize, black bullet, %150 spacing between items using "witemize"
%  \setbeamertemplate{itemize items}[circle]
%  \setbeamercolor{itemize item}{fg=black}
%  \setbeamercolor{enumerate item}{fg=black}
%  \setbeamercolor{itemize subitem}{fg=black}
%  \setbeamercolor{enumerate subitem}{fg=black}
%  \newenvironment{witemize}{\itemize\addtolength{\itemsep}{0.0\baselineskip}}{\enditemize}
%
%  % block, black over gray with no shadow
%  \setbeamertemplate{blocks}[rounded][shadow=false]
%  \setbeamercolor{block title}{fg=black,bg=gray!40}
%  \setbeamercolor{block body}{fg=black,bg=gray!10}
%
%  % frametitle, bold, black, centered
%  \setbeamertemplate{frametitle}[default][center]
%  \setbeamercolor{frametitle}{fg=black}
%  \setbeamerfont{frametitle}{shape=\bfseries}
%
%  % line spacing
%  \linespread{1.2}
%
%  \setlength{\parskip}{\smallskipamount}
%}

%% macros for letters

\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}

\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\rr}{{\mathrm{r}}}


%% macros for math notions and operators

\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}
\renewcommand{\SS}{{\mathbb{S}}}
\newcommand{\SSp}{\mathbb{S}_{+}}
\newcommand{\SSpp}{\mathbb{S}_{++}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\Sign}{\mathrm{Sign}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\vone}{{\mathbf{1}}}
\newcommand{\Null}{{\mathrm{Null}}}
\newcommand{\dist}{{\mathrm{dist}}}
\newcommand{\Co}{{\mathbf{Co}}}

\newcommand{\op}{{\mathrm{op}}} % subscript for operator norm
\newcommand{\opt}{{\mathrm{opt}}} % subscript for optimal solution
\newcommand{\supp}{{\mathrm{supp}}} % support
\newcommand{\Prob}{{\mathrm{Prob}}} % probability
\newcommand{\Diag}{{\mathrm{Diag}}} % vector -> diagonal matrix
\newcommand{\diag}{{\mathrm{diag}}} % matrix diagonal -> vector
\newcommand{\dom}{{\mathrm{dom}}} % domain
\newcommand{\grad}{{\nabla}}    % gradient
\newcommand{\tr}{{\mathrm{tr}}} % trace
\newcommand{\TV}{{\mathrm{TV}}} % total variation
\newcommand{\Proj}{{\mathrm{Proj}}}
\DeclareMathOperator{\shrink}{shrink} % shrinkage
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\mini}{minimize}
\DeclareMathOperator*{\maxi}{maximize}
\DeclareMathOperator*{\Min}{minimize}
\DeclareMathOperator*{\Max}{maximize}
\newcommand{\prox}{{\mathbf{prox}}}
\newcommand{\st}{{\quad\text{s.t.}~}}

%% macros for environments math equations

\newcommand{\MyFigure}[1]{../fig/#1}

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}

\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\bfl}{\begin{flushleft}}
\newcommand{\efl}{\end{flushleft}}

\newcommand{\bt}{\begin{tabbing}}
\newcommand{\et}{\end{tabbing}}

\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}

\newcommand{\beqs}{\begin{align*}} % no equation numbers
\newcommand{\eeqs}{\end{align*}}  % no equation numbers

%% macros for theorem-like environments

\newtheorem{theorem}{Theorem}
\newtheorem{condition}{Condition}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\newtheorem{proof}{Proof}
\newtheorem{proof*}{Proof}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}

% \newtheorem{example}[remark]{Example}




==> sec_RL2SL_notes.tex <==
% !TEX ROOT=./main.tex
\subsection{A discussion of prior works on reducing RL to SL.}
\label{sec:priworkRL2SL}
There are two main distinctions between supervised learning and reinforcement
learning. In supervised learning, the data distribution $\cD$ is static and training
samples are assumed to be sampled i.i.d. from $\cD$. On the contrary, 
the data distribution is dynamic in reinforcement learning since the RL agents 
collect data through interacting with the
environment. The data distribution is determined by both 
environment dynamics and the learning policy. The
policy keeps evolving during the learning process, therefore, the data distribution is dynamic in RL.  
Secondly, the training samples we collected
are not independently distributed due to the change of learning policy. 
These intrinsic difficulties of RL make the learning
algorithm unstable and sample-inefficient. However, if we review 
the state-of-the-arts in RL community, every algorithm eventually acquires the
policy, either explicitly or implicitly, which is a mapping from the current
state to an action or a probability distribution over the action space. Ultimately,
there exists a supervised learning equivalent to the RL problem, if the optimal
policies exists. The paradox is that it is almost impossible to construct this 
supervised learning equivalent on the fly, without knowing any optimal policy. Although 
what is the proper supervision still lingered in the RL community, pioneers 
have developed a set of insightful approaches to reduce RL into its SL 
counterpart over the past several decades. 
Roughly, we can classify the prior work into the following 
categories:
\begin{itemize}
  \item \textit{Expectation-Maximization (EM)}~\cite{dayan1997using,peters2007reinforcement,kober2009policy,abdolmaleki2018maximum}, etc.
  \item \textit{Entropy-Regularized RL (ERL)}~\cite{oh2018self,haarnoja2018soft}, etc.
  \item \textit{Preference based RL (PbRL)}~\cite{furnkranz2012preference,wirth2016model}, etc.
  \item \textit{Interactive Imitation Learning (IIL)}~\cite{daume2009search,ross2011reduction,sun2017deeply}, etc.
\end{itemize}

The early work in the EM track transfers objective by Jensen's 
inequality and the maximizing the lower bound of original objective, 
which resembles Expectation-Maximization procedure and provides policy improvement
guarantee. 
While pioneering at the time, these works typically focus on 
the simplified RL setting, such as in~\cite{dayan1997using} the reward function is 
not associated with the state or in~\cite{peters2008reinforcement}
the goal is to maximize the expected immediate reward and the state distribution is 
assumed to be fixed. Later on in~\cite{kober2009policy}, the authors extends the
EM framework from immediate reward into episodic return. 
Recent advance~\cite{abdolmaleki2018maximum} utilizes the EM-framework
on a relative entropy objective, which adds a parameter prior as regularization.
As mentioned in the paper, the evaluation step using \textit{Retrace}~\cite{munos2016safe}
can be unstable even with linear function approximation~\cite{touati2017convergent}. In fact,
the evaluation step in EM track typically involves on-policy evaluation, 
which is one difficulty shared for any policy gradient methods. One of the main motivation that we
want to transfer the RL into a supervised learning task is the off-policy learning enable
sample efficiency. 
\begin{itemize}
  \item on-policy [page 4 in~\cite{dayan1997using}] 
  \item on-policy E-step in Alg 1. the samples need to corresponds to current parameters $\theta$~\cite{peters2008reinforcement}]. Although the reward-weighted regression is supervised learning, see eq 12 in Alg 1. the E-step is on-policy. 
  \item \cite{kober2009policy} \{This algorithm formulates
the policy optimization as an Expectation-Maximization
problem to avoid the need to manually choose learning
rate, and the method is guaranteed to converge to a locally optimal solution (copy from~\cite{duan2016benchmarking})\}.  This is a return-weighted regression problem. on-policy due to the 
estimate step in Alg 1. The reweighted is using unbiased estimate of return of current parameter $\theta$.
\item E-step is originally on-policy~\cite{abdolmaleki2018maximum}. off-policy cannot be used without importance sampling. see eq 13 and foot note 2 in~\cite{abdolmaleki2018maximum}.
\end{itemize}

To achieve off-policy learning, Soft Actor-Critic
~\cite{haarnoja2018soft} was proposed to enable sample-efficient and 
faster convergence under the framework of entropy-regularized RL. 
It is able to converge to the optimal policy that optimizes the long term reward
along with policy entropy. It is an efficient way to model the suboptimal behavior
and empirically it is able to learn a reasonable policy. However, the discrepancy
between two objectives are not clear. In~\cite{oh2018self}, 
this work share similarity to our work in terms of 
the method we collecting the samples. They collect good samples based on the 
past experience and then conduct the imitation learning w.r.t those good samples. 
However, we differentiate at how do we look at the problem theoretically. This self-imitation
learning procedure was eventually connected to lower-bound-soft-Q-learning, which belongs to 
entropy-regularized reinforcement learning. We comment that, there is a trade-off between collecting
good samples and modeling suboptimal behaviors. 
The more strict requirement we have on the samples
collected we have less chance to hit the samples while we are more close to imitate the optimal behavior.
% as shown in Figure~\ref{fig:sltf}. 
The concrete study on this will be a follow up work. 

Preference based RL has arisen as an alternative approach to cast RL as supervised learning, 
where the reward signal is unknown while the trajectory preference is
assumed to be able to solicit from the experts~\cite{wirth2016model,furnkranz2012preference}. 

From the track of interactive imitation learning, 
initial representative works such as~\cite{ross2010efficient,ross2011reduction} 
% daume2009search Search-based structured prediction  
firstly pointed out the main discrepancy between imitation learning and reinforcement learning
is the i.i.d. assumption does not hold and provides \textsc{SMILe}~\cite{ross2010efficient} and
\textsc{DAgger}~\cite{ross2011reduction} to overcome the distribution mismatch. 
The theorem 2.1 in 
~\cite{ross2010efficient} firstly analyzed if the learned policy fail to imitate the expert
with certain probability, what is the performance drop comparing to the expert. 
While the
theorem seems to resemble the long term performance theorem~\ref{th:ltpt}, it is actually 
consider the learning policy is trained through the state distribution induced by the expert, instead
of state-action distribution as we did in Theorem~\ref{th:ltpt}. Their theorem thus
may be more applicable to the situation where an interactive procedure is needed, such as 
querying the expert during the training process. On the contrary, we focus on directly applying
supervised learning approach without having access to the expert to label the data. The optimal
state-action pairs are collected during exploration and conducting supervised learning on
the replay buffer will provide a performance guarantee in terms of long term expected reward. 
Concurrently, a resemble of theorem 2.1 in~\cite{ross2010efficient} is Theorem 1 in~\cite{syed2010reduction}, the authors reduce the apprenticeship learning to classification, under the
assumption that the apprentice policy is deterministic and the misclassification rate at
all time steps is bounded, which we do not make. 
Within the IIL track, later on 
the \textsc{AggreVaTe}~\cite{ross2014reinforcement} was proposed to incorporate the
information of action costs to facilitate imitation learning, and a differentiable version 
called \textsc{AggreVaTeD}~\cite{sun2017deeply} was recently developed 
which achieved impressive empirical results. 

In conclusion, our method approaches the problem of reducing RL to SL from a different prospective
than all prior works mentioned. With our construction from RL to SL, the samples collected in replay buffer 
can satisfy the i.i.d. assumption exactly since the state action pairs are sampled from the data distribution
of UNOP. 
A summary of similarity and discrepancy between our method 
the current best method in each category is shown in the Table~\ref{tb:rl2sl}.
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|} \hline
  \multicolumn{1}{|l|}{Methods} &  \multicolumn{1}{l|}{Objective} & \multicolumn{1}{l|}{Action} &  \multicolumn{1}{l|}{Optimal}& \multicolumn{1}{l|}{Off-Policy} & \multicolumn{1}{l|}{No Oracle} \\ \hline \hline 
   \multicolumn{1}{|p{1cm}|}{ EM} 
 & \multicolumn{1}{p{1cm}|}{ \checkmark } 
 & \multicolumn{1}{p{1cm}|}{ \checkmark }
 & \multicolumn{1}{p{1cm}|}{ \xmark}
 & \multicolumn{1}{p{1cm}|}{ \xmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark} \\ \hline
% 
   \multicolumn{1}{|p{1cm}|}{ ERL} 
 & \multicolumn{1}{p{1cm}|}{ \xmark } 
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark} \\ \hline
% 
   \multicolumn{1}{|p{1cm}|}{ IIL} 
  & \multicolumn{1}{p{1cm}|}{ \checkmark } 
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \xmark} \\ \hline
%
   \multicolumn{1}{|p{1cm}|}{ PbRL} 
 & \multicolumn{1}{p{1cm}|}{ \checkmark } 
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \xmark} \\ \hline
    \multicolumn{1}{|p{1cm}|}{ RPG} 
 & \multicolumn{1}{p{1cm}|}{ \checkmark } 
 & \multicolumn{1}{p{1cm}|}{ \xmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark}
 & \multicolumn{1}{p{1cm}|}{ \checkmark} \\ \hline
\end{tabular}
\caption{A comparison with prior work on reducing RL to SL. The \textit{objective} column denotes whether
the goal is to maximize long term reward.  The \textit{Action} column denotes whether the 
method is applicable for both continuous action space and discrete action space. The \textit{Optimal}
denotes whether the algorithms model the optimal policy. The \textit{Off-Policy} column denotes
if the algorithm enable off-policy learning. The \textit{No Oracle} column 
denotes if the algorithms need to access to certain type of oracle.}
\label{tb:rl2sl}
\end{table*}  
 

% \begin{figure*}
% \centering
%   \includegraphics[width=0.8\textwidth]{fig/SLtradeoff.pdf}
%   \caption{The trade off between modeling optimal behavior and the exploration efficiency. SIL~\cite{oh2018self}, SAC~\cite{haarnoja2018soft}, MPO~\cite{abdolmaleki2018maximum} may not be modeling suboptimal.}
%   \label{fig:sltf}
% \end{figure*}


==> sec_RL_sample_complexityproof_loose.tex <==
\subsection{The proof of Theorem~\ref{th:rlgp}}
\label{sec:app:samplecomplex-v1}

\begin{theorem}[Generalization Performance]
Given a MDP where the UNOP (Def~\ref{def:uop}) is deterministic, let $|\cH|$ denotes the size of hypothesis space, and let $\delta, \gamma$ be fixed, 
$(\min_{h\in\cH}\epsilon(h))  + 2\gamma = \eta$. If we want the following inequality holds with probability at least $1 - \delta$,
\begin{align}
& \sum_{\tau} p_{\theta}(\tau)r(\tau)  \geq \sum_{\tau} p_{\theta}(\tau)w(\tau) = \sum_{\tau\in \cT} p_{\theta}(\tau)w(\tau)\geq L_p\\
& \text{where } \nonumber \\
& L_{p} = |\cT|\left(\Pi_{\tau\in \cT} p_d(\tau)\right)^{\frac{1}{|\cT|}}\exp((1-m)(\frac{3}{2}\eta + \log2)T) = O(e^{- m \eta T})
\end{align}
the number of state action pairs (training sample size $n$) from the optimal uniformly policy needs to satisfy:
    \begin{equation}
      n \geq \frac{1}{2\gamma^2} \log\frac{2|\cH|}{\delta}
    \end{equation}
where $p_d(\tau) = p(s_1)\Pi_{t=1}^{T}p(s_{t+1}|s_{t}, a_{t})$ denotes the environment dynamics and 
it can not be improved by our learning algorithm. 
\label{th:rlgp}
\end{theorem}
 
\begin{corollary}[The range of lower bound]
  The lower bound $L_p \in (0, 2^{T(1-m)}\bar{p}_d|\cT|]$, where
  $\bar{p}_d = \frac{1}{|\cT|}\sum_{\tau\in \cT} p_d(\tau)$ is the averaged
  dynamics of all near-optimal trajectories.
  \label{cor:tlb}
\end{corollary}


\begin{proof}
The proof mainly establishes on the proof for long term performance theorem~\ref{th:ltpt}
and connects the generalization bound in PAC framework to the lower bound of return.
\begin{align}
 % & \sum_{\tau} p_{\theta}(\tau) w(\tau) \\
 & \log (\frac{1}{|\cT|}\sum_{\tau\in \cT} p_{\theta}(\tau)w(\tau) ) \geq  \frac{1}{|\cT|}\sum_{\tau\in \cT}  \log p_{\theta}(\tau)w(\tau)\\
 \Leftrightarrow & \sum_{\tau\in \cT} p_{\theta}(\tau)w(\tau)  \geq |\cT| \exp(\frac{1}{|\cT|}\sum_{\tau\in \cT}  \log p_{\theta}(\tau)w(\tau)) \\
 &  \text{  denote } F = \sum_{\tau} p_{\theta}(\tau)w(\tau) = \sum_{\tau\in \cT} p_{\theta}(\tau)w(\tau) \nonumber \\
 \Leftrightarrow F & \geq |\cT| \exp(\frac{1}{|\cT|}\sum_{\tau\in \cT}  \log p_{\theta}(\tau)w(\tau)) \\
  % &= |\cT| \exp(\frac{1}{|\cT|}\sum_{\tau\in \cT}  \log p_{\theta}(\tau)w(\tau)) \\  
  &= |\cT| \exp\left( \frac{1}{|\cT|}\sum_{\tau\in \cT} \left(\log p(s_1) + \sum_{t=1}^{T}\log p(s_{t+1}|s_{t}, a_{t})+ \sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t) + \log w(\tau) \right) \right) \\
  & \because w(\tau)= 1, \ \forall \tau \in \cT, s_t = s(\tau, t), a_t=a(\tau, t), t =1,\dots, T \\
  &= |\cT| \exp\left( \frac{1}{|\cT|}\sum_{\tau\in \cT} \left(\log p(s_1) + \sum_{t=1}^{T}\log p(s_{t+1}|s_{t}, a_{t})+ \sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t) \right) \right) \\
  &= |\cT| \exp\left( \frac{1}{|\cT|}\sum_{\tau\in \cT} (\log p(s_1) + \sum_{t=1}^{T}\log p(s_{t+1}|s_{t}, a_{t}))\right)\exp\left( \frac{1}{|\cT|}\sum_{\tau\in \cT}(\sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t)) \right) \\
  & \text{ Denote the dynamics of a trajectory as } p_d(\tau) = p(s_1)\Pi_{t=1}^{T}p(s_{t+1}|s_{t}, a_{t})  \nonumber\\
  & \text{ Notice that } p_d(\tau) \text{ is environment dynamics, which is fixed given a specific MDP.} \nonumber\\
  \Leftrightarrow  F & \geq |\cT| \exp\left( \frac{1}{|\cT|}\sum_{\tau\in \cT}\log p_d(\tau)\right)\exp\left( \frac{1}{|\cT|}\sum_{\tau\in \cT}(\sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t)) \right) \\
  & = |\cT|\left(\Pi_{\tau\in \cT} p_d(\tau)\right)^{\frac{1}{|\cT|}}\exp\left( \frac{1}{|\cT|T}\sum_{\tau\in \cT}(\sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t)) T \right) \\
  & \text{Use the same reasoning from \eq{\ref{eq:ltpt:sumtraj}} to \eq{\ref{eq:ltpt:slapp}}. }\\
  & = |\cT|\left(\Pi_{\tau\in \cT} p_d(\tau)\right)^{\frac{1}{|\cT|}}\exp\left( T\sum_{s,a} p_{\pi_*}(s, a) \log\pi_{\theta}(a|s) \right) \\
  & = |\cT|\left(\Pi_{\tau\in \cT} p_d(\tau)\right)^{\frac{1}{|\cT|}}\exp(TL) \\
  & \text{Apply Corollary~\ref{cor:rppg} and denote } L = \sum_{s,a} p_{\pi_*}(s, a) \log\pi_{\theta}(a|s). \nonumber\\
  & L \text{ is the only term that is related to the policy parameter } \theta \nonumber \\
  L & = \sum_{s,a} p_{\pi_*}(s, a)\log(\Pi_{j\neq i, j=1}^m p_{ij} )\\
  & = - \sum_{s, a_i}p_{\pi_*}(s, a_i)\sum_{j\neq i, j=1}^m\log (1 + e^{Q_{ji}})\\
  & \text{Use Taylor expansion: } \log(1+ e^x) = \log2 + \frac{1}{2}(x) + \cO(x^2)\\
  &= -\sum_{s, a_i}p_{\pi_*}(s, a_i)\sum_{j\neq i, j=1}^m (\log2 + \frac{1}{2}Q_{ji}+ \cO(O_{ij}^2)) \\
  % &\approx - \sum_{s, a_i}p_{\pi_*}(s, a_i)((m-1)\log2 + \sum_{j\neq i, j=1}^m \frac{1}{2}(Q_{i} - Q_j)) \text{ \lkxcom{?Ignoring} the high order term here.} \\
  & = \sum_{s, a_i}p_{\pi_*}(s, a_i)\sum_{j\neq i, j=1}^m [\frac{1}{2}(Q_{i} - Q_j) - \cO(O_{ij}^2)] - (m-1)\log2\\
  % & = \sum_{s, a_i}p_{\pi_*}(s, a_i)\sum_{j=1,j\neq i}^{m} \max (0 , \text{margin} + Q(s, a_j) - Q(s,  a_{i}) )
  &\text{Given } h = \pi_\theta, \text{misclassified state action pairs set } U_w = \{s, a| h(s)\neq a, (s,a)\sim p_*(s,a)\}\\
  &\text{Apply Lemma~\ref{lemma:samplecomplexiy}, the probability that the classifier is correctly classify the state is at least } 1 - \eta.\\
  L & = \sum_{(s, a_i) \notin U_w}p_{\pi_*}(s, a_i)\sum_{j\neq i, j=1}^m [\frac{1}{2}(Q_i - Q_j) - \cO(O_{ij}^2)] \\
   & + \sum_{(s, a_i) \in U_w}p_{\pi_*}(s, a_i)\sum_{j\neq i, j=1}^m [\frac{1}{2}(Q_i - Q_j) - \cO(O_{ij}^2)]- (m-1)\log2 \\
  & \text{ the first term corresponds to the correctly classified states.}\\
  & \because Q_{ij} \leq c_q < 1, \therefore Q_{ij} > O(Q_{ij}^2), \forall (s, a_i) \in U_w. \text{ we drop the first term.}\\
& \geq \sum_{(s, a_i) \in U_w}p_{\pi_*}(s, a_i)\sum_{j\neq i, j=1}^m [\frac{1}{2}(Q_i - Q_j) - \cO(O_{ij}^2)]- (m-1)\log2 \\
& \because O(Q_{ij}^2)\leq c_q^2 < 1, \therefore - O(Q_{ij}^2) \geq -c_q^2  > - 1\\
& \geq \sum_{(s, a_i) \in U_w}p_{\pi_*}(s, a_i)\sum_{j\neq i, j=1}^m [\frac{1}{2}(Q_i - Q_j) - c_q^2]- (m-1)\log2 \\
& \because Q_{ij}\leq c_q, \therefore Q_{ij} \geq -c_q >  - 1\\
    & \geq \sum_{(s, a_i) \in U_w}p_{\pi_*}(s, a_i)\sum_{j\neq i, j=1}^m [-\frac{1}{2}c_q - c_q^2]- (m-1)\log2 \\
    & \geq -\sum_{(s, a_i) \in U_w}p_{\pi_*}(s, a_i) (\frac{1}{2}c_q + c_q^2)(m-1)  + (1-m)\log2\\
    & \text{ Apply Lemma~\ref{lemma:samplecomplexiy}} \sum_{(s, a_i) \in U_w}p_{\pi_*}(s, a_i) \leq \eta \ \rightarrow - \sum_{(s, a_i) \in U_w}p_{\pi_*}(s, a_i) \geq -\eta  + (1-m)\log2\\
    & \geq -(m-1) (\eta(\frac{1}{2}c_q + c_q^2) +\log2) \text{ Use } c_q < 1\\
    & \geq -(m-1) (\frac{3}{2}c_q\eta + \log2)\\
   \therefore F & \geq |\cT|\left(\Pi_{\tau\in \cT} p_d(\tau)\right)^{\frac{1}{|\cT|}}\exp((1-m)(\frac{3}{2}c_q\eta + \log2)T) \\
   &  \geq |\cT|\left(\Pi_{\tau\in \cT} p_d(\tau)\right)^{\frac{1}{|\cT|}}\exp((1-m)(\frac{3}{2}\eta + \log2)T) = L_p
\end{align}


From generalization performance to sample complexity: 
\begin{align*}
  & \mathrm{Set }\  L_p = R_{\max} - \epsilon, D = |\cT|\left(\Pi_{\tau\in \cT} p_d(\tau)\right)^{\frac{1}{|\cT|}}  \\
  &\Rightarrow R_{\max} - \epsilon = D \exp((1-m)(\frac{3}{2}\eta + \log2)T)\\
    &\Rightarrow  \frac{3}{2}\eta + \log2 = \frac{\ln \frac{R_{\max} - \epsilon}{D}}{T(1-m)} \\
    &\Rightarrow  \eta = \frac{3\ln \frac{R_{\max} - \epsilon}{D}}{2T(1-m)} - \frac{2}{3}\log2  \\
    &\Rightarrow \gamma = \frac{\eta - \epsilon_{\min}}{2} = \frac{\ln \frac{R_{\max} - \epsilon}{D}}{3T(1-m)} - \frac{1}{3}\log2 - \frac{\epsilon_{\min}}{2} \\
    &\because n \geq \frac{1}{2\gamma^2} \log\frac{2|\cH|}{\delta}\\
    &\therefore n \geq \frac{1}{2\left(\frac{\ln \frac{1 - \epsilon}{D}}{3T(1-m)} - \frac{1}{3}\log2 - \frac{\epsilon_{\min}}{2}\right)^2} \log\frac{2|\cH|}{\delta} \\
    &\because  m > 1 \\
    &n \geq \frac{1}{2\left(\frac{\ln \frac{D}{1 - \epsilon}}{3T(m-1)} - \frac{1}{3}\log2 - \frac{\epsilon_{\min}}{2}\right)^2} \log\frac{2|\cH|}{\delta}
\end{align*}
\end{proof}

==> sec_alg1.tex <==
% !TEX ROOT=./main.tex
\begin{algorithm}[h!]\small
\begin{algorithmic}[1]
\REQUIRE The near-optimal trajectory reward threshold $c$, the number of maximal training episodes $N_{max}$.
Maximum number of time steps in each episode $T$, and batch size $b$.  %The exploration threshold $t_e$
\WHILE { episode $< N_{\max}$}
\REPEAT
\STATE Retrieve state $s_t$ and sample action $a_t$ by the specified exploration agent 
       (can be random, $\epsilon$-greedy, or any RL algorithms).
\STATE Collect the experience $e_t = (s_t, a_t, r_t, s_{t+1})$ and store to the replay buffer.
\STATE $t= t +1$
\IF {t \% update step == 0}
\STATE Sample a batch of experience $\{e_j\}_{j=1}^b$ from the near-optimal replay buffer.
\STATE Update $\pi_{\theta}$ based on the hinge loss~\eq{\ref{eq:rankingv2}} for RPG.
\STATE Update exploration agent using samples from regular replay buffer (In simple MDPs such as 
\textsc{Pong} where we access to near-optimal trajectory frequently, we can use near-optimal replay buffer 
to update exploration agent).
\ENDIF
\UNTIL{terminal $s_t$ or $t- t_{\text{start}} >=T$} % t_max explained in 4.3 2nd
\IF {return $\sum_{t=1}^Tr_t \geq c$}
\STATE Take the near-optimal trajectory $e_t, t=1,...,T$ in the latest episode 
from the regular replay buffer into near-optimal replay buffer.
\ENDIF
\IF {t \% evaluation step == 0}
\STATE Evaluate the RPG agent by greedily choosing the action. If the best performance is reached, then stop training.
\ENDIF
\ENDWHILE
\end{algorithmic}
\caption{Off-Policy Learning for Ranking Policy Gradient (RPG)}% $S$ = cA3C($\theta, \Theta_v$
\label{alg:rankingrl}
\end{algorithm}


==> sec_exp_motivating.tex <==
% !TEX ROOT=./main.tex
% \subsection{A Motivating Example}
% Theory is an approximation of reality. To understand what are the potential
% discrepancies and alignments between the proposed theorems and practice, we designed
% a relative simplified motivating example to exam the effectiveness of ranking 
% policy gradient (RPG) and evolving policy gradient (EPG). 

% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.3\textwidth]{fig/toy_example.png}
% \label{fig:label1}
% \caption{A illustration of game board of our toy example using Pommerman environment.}
% \end{figure}

\begin{figure}
\centering
% \includegraphics[width=0.5\textwidth]{fig/fiverandomseedave_rankingvspervsregular.png}
\includegraphics[width=0.5\textwidth]{fig/toy_results.pdf}
% from notebook: /notebooks/pommerman/notebooks/playground_test.ipynb flag=fiverepreat
% /home/linkaixi/Dropbox/pommerman/toy/runner_oneshot.py
\caption{The training curves of double DQN (shown in the red curve), double DQN with prioritized experience
replay (shown in the green curve), one-shot imitation learning (shown in the yellow curve),
 and the proposed RPG algorithm (shown in the blue curve.) 
 1Shot denotes the performance of RPG trained with one optimal trajectory. 
All results are averaged over random seeds from 1 to 5. The $x$-axis indicates the training episodes and the $y$-axis is the
long-term episodic reward during each training episode.}
\label{fig:rpg_rank_toy}
\end{figure}
In this section, we design a toy example to illustrate the possible reason that RPG is 
more sample efficient than DQN variants.
The toy example is designed as follows.  We want to train an agent playing against a static agent (a agent
that never move) in the Pommerman environment~\citep{resnick2018pommerman}. %as shown in Figure~\ref{fig:label1}.
 The goal is to kill the static agent as soon as 
possible by placing a bomb beside the opponent, and avoid being killed by the bomb.
We briefly summarize the main features of the environment as follows, for more details
please refer to the white paper~\citep{resnick2018pommerman}. 
\begin{itemize}
	\item State: The agent observes part of the board including opponents' position,
	bombs' positions and in how many time steps the bomb will explode. The initial states
	of the two agents are fixed. 
	\item Action: The agent has six actions including moving towards four directions, staying
	in the current position or placing a bomb. 
	\item Reward: The agent receives a $-2$ reward for each time step, in order to encourage 
	killing the enemy as soon as possible. A $+100$ reward is given for killing the enemy and $-100$ reward for being killed. We empirically designed this reward function to facilitate 
	the learning procedure.
	\item Horizon: we limit the time horizon to be 100 time step.
\end{itemize}

% \textbf{Does it work?}
% Firstly, we would like to show whether the proposed algorithm is  a sample
% efficient algorithm compared to other off-policy methods.  Our baselines is
% double DQN~\citep{van2016deep} with regular experience replay and prioritized
% experience replay. For fair comparison, we first tune a good $\epsilon$-greedy 
% (linearly annealed from 1 to 0.1 at first 20000 time steps.)
% strategy for double DQN and directly use the same strategy with RPG. All
% three methods use the exact same neural network architecture and feature
% design. The result is shown in Figure~\ref{fig:rpg_vs_epg}. 

\textbf{One-shot imitation learning with RPG}: 
Given that the agent already experienced an optimal trajectory, 
RPG agent can quickly master the lessons learned and 
follow it repeatedly, rather than exploring all kinds of possibilities in the entire
state-action space. Therefore, the foundation of RPG is actually one-shot imitation 
learning. The performance of one-shot imitation learning is shown as the yellow curve
in Figure~\ref{fig:rpg_rank_toy}.

% \textbf{How does it work?}
% The TP (Def~\ref{def:PI}) stabilize and accelerate the performance of policy gradient method and
% RPG further improve the sample efficiency. In Figure~\ref{fig:rpg_vs_epg}, we show the 
% results of RPG and EPG.

% \begin{figure}
% \centering
% \includegraphics[width=0.5\textwidth]{fig/toy_VPGRPG_exp.pdf}
% % from notebook: /notebooks/pommerman/notebooks/playground_test.ipynb flag=fiverepreatVPGRPG
% % /home/linkaixi/Dropbox/pommerman/toy/runer_central_ranking.py
% \label{fig:rpg_vs_epg}
% \caption{The training curves of EPG (shown in a red curve) and the proposed RPG algorithm (shown in blue curve.) For RPG, we random explore the environment in first 2000 time steps and then greedy chose 
% the action. We train the RPG model in first 5000 time steps.
% All results are averaged over random seeds from 1 to 5. The x-axis is the training episodes and the 
% y-axis is the long term episodic reward for during each training episode.}
% \end{figure}



==> sec_method_backup.tex <==
% !TEX ROOT=./main.tex

\begin{lemma}[Optimal Sample Rate, proof and conclusion is not correct.]
Given a stationary policy $\pi_{\theta}$,	$p_{\theta}(\tau), \forall \tau \in \cT$ is 
the probability that we hit each trajectory in the optimal trajectory set, 
we denote the $\xi_m = \min_{\tau \in \cT} p_{\theta}(\tau)$, 
$\xi_s =\sum_{\tau \in \cT}  p_{\theta}(\tau)$. 
In the first $k$ episodes, with probability at least
\begin{align}
\sum_{i=n'}^{ \min\{|\cT|, k\}} C_{k}^i C_{|\cT|}^i\xi_m^i (1-\xi_s)^{k-i}	
\end{align}
we can collect
at least $Tn'$ optimal state action pairs. We denote the number of
combinations choosing $i$ items from $k$ as $ C_{k}^i  = \frac{k!}{i! (k - i)!}$.
\label{lemma:osr}
\end{lemma}
\begin{proof}
In total, suppose there are $B$ optimal trajectories.
The probability of hitting at least $n'$ optimal trajectories in the first
 $k$ episodes (denoted as $P_{\geq n'}$)is given as follows:
 \begin{align}
 	P_{\geq n'} = \sum_{i=n'}^{\min\{|\cT|,k\}} P_{i}
 \end{align} 
 where $P_{i}$ denotes the probability of hitting exactly optimal
 trajectories in first $k$ episodes.  $P_{i}$ can be computed as follows:
 \begin{align}
 	 P_{i} &= C_{k}^i(1- \xi_s)^{k - i}\left(\overbrace{
 	 p_{\theta}(\tau_{j_1})p_{\theta}(\tau_{j_2})\dots p_{\theta}(\tau_{j_i})
 	 + \dots + p_{\theta}(\tau_{j_1})p_{\theta}(\tau_{j_2})\dots p_{\theta}(\tau_{j_i})}^{C_{|\cT|}^i \text{ combinations}} \right) \\
 	 &\geq C_{k}^i(1- \xi_s)^{k - i}\left( C_{|\cT|}^i \xi_m^i\right)
 \end{align} 
Therefore, 

 \begin{align}
 	P_{\geq n'} &= \sum_{i=n'}^{\min\{|\cT|,k\}} P_{i}\\
 	 &= \sum_{i=n'}^{\min\{|\cT|,k\}}C_{|\cT|}^i C_{k}^i\xi_m^i(1- \xi_s)^{k - i}
 \end{align} 
For example, if we draw $10$ episodes, there are in total $3$ optimal trajectories
($\tau_1, \tau_2, \tau_3$). The probability we hit $2$ optimal trajectories in first
$3$ iterations is:
\begin{align}
	p_2 =&  C_{10}^2 (1 - \xi_s)^8 (p_{\theta}(\tau_1)p_{\theta}(\tau_2)+ p_{\theta}(\tau_1)p_{\theta}(\tau_3)+ p_{\theta}(\tau_3)p_{\theta}(\tau_2))\\
\geq&  C_{10}^2 (1 - \xi_s)^8 (\xi_m^2*3)\\
= &  C_{10}^2 (1 - \xi_s)^8 (\xi_m^2*C_3^2)
\end{align}
\end{proof}


Tonelli's theorem if $f_n(x)\geq 0 \forall n, x$, then $\int \sum_n f_n(x) = \sum_n \int f_n(x) dx$

\lkxthink{
\begin{itemize}
	\item Why Hinge loss is more sample-efficient than sigmoid (which is used everywhere in policy gradient/actor method)? what's the assumption of hinge loss.
\end{itemize}}


\begin{remark}
\textbf{We don't have any assumption on the state distribution of $d(s_0)$, 
this is essential to off-policy learning, since it can come from any policy!
Which means during the training, suppose the current policy is $\theta_k$, given any state action pairs $(s_0, a_0)$, collected by other policy, we can utilize it improve the current policy, since we can assume what if $\theta_k$ encounter this state action pair, and simply improve the policy $\theta_k$ by PEPGT~\ref{th:pEPGT}}
\end{remark}

To achieve off-policy learning, we need to consider the gradient of evolving return 
$\vE_{\{\pi_i\}_{i=0}^{T}, \vP}[R_0]$ with respect to the starting policy $\pi_0$. Suppose (unless other specified!)
$\pi_0=\pi_{\theta}$ is parameterized by $\theta$. Then similar to the policy gradient theorem, we have the gradient under policy $\pi_0$ as follows:
\begin{align}
\grad_{\theta}\vE_{\{\pi_i\}_{i=0}^{T}, \vP}[\cR_0] = \int d(s_0) \pi_{\theta}(s_0, a_0)\grad_{\theta}\log \pi_{\theta} (s_0, a_0) \left(r(s_0, a_0) + \gamma\vE_{\{\pi_i\}_{i=1}^{T}, \vP}[\cR_1]\right) ds_0 da_0
\label{eq:true_gradient}
\end{align}


We define the return of a series of evolving policies starting at time step $t=0$ as following:
\begin{align}
 & \vE_{\{\pi_i\}_{i=0}^{T}, \vP}[\cR_0]\\
 &= \int d(s_0)\pi_0(s_0, a_0)p_{s_0s_{1}}^{a_0} \pi_{1}(s_1, a_1)...P_{s_{T-1},s_T}^{a_{T-1}} \sum_{i=0}^T \gamma^{i}r(s_i, a_i) ds_Tda_{T-1}d\pi_{T-1}...da_1d\pi_1ds_1da_0ds_0 \\
 &= \int d(s_0)\pi_0(s_0, a_0) \left(r(s_0, a_0) + \gamma\vE_{\{\pi_i\}_{i=1}^{T}, \vP}[\cR_1]\right)da_0ds_0 
\end{align}


\lkxcom{keep this in mind: the key is to select the good trajectories only.
essentially that's why it can be off-policy.}


\lkxthink{ off-policy procedure.
\begin{itemize}
	\item Current policy $\theta_k$,
	\item sample pairs $(s_t, a_t, \cR_t(\{\pi_i\}_{i=t}^T))$ from experience replay buffer.
	\item Use this sample pair collected by other policy to train the policy $\theta_k$ by updating gradient $\grad_{\theta_k} \log\pi_{\theta_k}(a_t|s_t) \cR_t(\pi_t)$. 
	\item Notice that $\theta_k \neq \theta_0$
\end{itemize}}

\lkxcom{\textbf{[The remaining building blocks]}
\begin{itemize}
	\item A convergence proof see last theorem in paper~\cite{sutton2000policy} for hint
	\item Policy improve theorem
\end{itemize}}


\begin{align}
	&\argmax_{\theta} \sum_{\tau} p_{\theta}(\tau) w(\tau)\\
% = & \argmax_{\theta} \sum_{\tau \in \cT} p(\tau) \\
& \text{we assume there is one optimal policy and } p_{\theta}(\tau)>0, \forall \tau \in \cT\\
= &  \argmax_{\theta} \sum_{\tau\in\cT}  \log(p_{\theta}(\tau))\\
=&\argmax_{\theta} \sum_{\tau} \log(p(s_1)\Pi_{t=1}^{T}(\pi_{\theta}(a_t|s_t)p(s_{t+1}|s_{t}, a_{t}))w(\tau))\\
=&\argmax_{\theta} \sum_{\tau} \log(p(s_1)(\Pi_{t=1}^{T}\pi_{\theta}(a_t|s_t)) \\ 
 & \hspace{2.8cm}(\Pi_{t=1}^{T}p(s_{t+1}|s_{t}, a_{t}))w(\tau))\\
=&\argmax_{\theta} \sum_{\tau} \log(p(s_1)(\Pi_{t=1}^{T}\pi_{\theta}(a_t|s_t)) \\ 
 & \hspace{2.8cm}(\Pi_{t=1}^{T}p(s_{t+1}|s_{t}, a_{t}))w(\tau)^T)\\
 =&\argmax_{\theta} \sum_{\tau} \log\left(p(s_1)(\Pi_{t=1}^{T}\pi_{\theta}(a_t|s_t))(\Pi_{t=1}^{T}p(s_{t+1}|s_{t}, a_{t})w(\tau))\right)\\
=& \argmax_{\theta} \sum_{\tau} \left( \log p(s_1) + \sum_{t=1}^{T}\log p(s_{t+1}|s_{t}, a_{t})+ \sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t)w(\tau) \right)\\
=& \argmax_{\theta} \frac{1}{|\tau|} \sum_{\tau} \sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t)w(\tau)\\
=& \argmax_{\theta} \frac{1}{|\tau|T} \sum_{\tau} \sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t)w(\tau) \\
=& \argmax_{\theta} \frac{1}{|\tau|} \sum_{\tau}\frac{1}{T} \sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t)w(\tau) \\
=&\argmax_{\theta}  \sum_{\tau } p_{\pi_*}(\tau) \frac{1}{T} \left(\sum_{t=1}^{T}\log\pi_{\theta}(a_t|s_t)w(\tau)\right) \\
=&\argmax_{\theta}  \sum_{\tau } p_{\pi_*}(\tau)   \sum_{s, a} p(s|\tau)\pi_*(a|s)\log\pi_{\theta}(a_t=a|s_t=s)w(\tau) \\
& \text{The 2nd sum is sum over all possible state action pairs. }\nonumber\\
& \text{s, a represents a specific state action pair.}\nonumber\\
=&\argmax_{\theta}  \sum_{\tau}  p_{\pi_*}(\tau) w(\tau)\sum_{s,a} p(s, a|\tau) \log\pi_{\theta}(a|s) \\
=&\argmax_{\theta}  \sum_{\tau }\sum_{s,a}  p_{\pi_*}(\tau)w(\tau) p(s, a|\tau) \log\pi_{\theta}(a|s) \\
=&\argmax_{\theta}  \sum_{s,a} \sum_{\tau} p_{\pi_*}(\tau) w(\tau)p(s, a|\tau) \log\pi_{\theta}(a|s) \\
=&\argmax_{\theta}  \sum_{s,a} \sum_{\tau} p_{\pi_*}(\tau) p(s, a|\tau) \log\pi_{\theta}(a|s) \\
& \text{based on the definition of performance indicator, } p_{\pi_*}(\tau) = 0, \text{if and only if } w(\tau) =0 \\
& \text{the above is established on transition dynamic can be zero. if optimal action is taken, zero probability to wrong states.}\\
& \text{which means, the probability of bad trajectory under optimal policy can be zero. otherwise we can find 
another policy, \lkxcom{this is an assumption}}\\
=&\argmax_{\theta}  \sum_{s,a} p_{\pi_*}(s, a) \log\pi_{\theta}(a|s) 
\end{align}

==> sec_optimalpolicy.tex <==
% !TEX ROOT=./main.tex

\section{Optimal policy existence}
\lkxcom{
Current progress of optimal policy: 
}
\begin{itemize}
	\item For deterministic task, the proper policy [Def 2.1 in~\cite{bertsekas1995neuro}] means that there exists an optimal trajectory.
	\item proper policy is a stationary policy that has positive probability
	to reach the terminal state. I can transfer this to the probability
	to hit the optimal trajectory.
\end{itemize}

\lkxcom{The policy improvement theorem may not be suitable in this framework, 
based on the value function. May be try to approach to it from the supervised approach.}





==> sec_relatedwork_old.tex <==
% !TEX ROOT=./main.tex

\section{Related works}



% related work to Sample efficient RL. policy gradient theorem off policy learning.
\noindent\textit{Sample Efficiency.}
The sample efficient reinforcement learning can be roughly divided into two categories.
The first category includes variants of $Q$-learning~\cite{mnih2015human,schaul2015prioritized,van2016deep,hessel2017rainbow}. The main advantage of $Q$-learning methods
is the use of off-policy learning, which is essential towards sample efficiency.
They are theoretically applicable and empirically successful.  
The representative DQN~\cite{mnih2015human} introduced deep neural network in $Q$-learning,
They proposed target network and experience replay to stabilize the training and firstly
enable the reinforcement learning to reach the human-level performance in complicated video games.
Prioritized experience replay~\cite{schaul2015prioritized} optimizes the sampling strategy from replay buffer 
using TD error, which largely accelerated the sample efficiency. 
\textsc{Rainbow}~\cite{hessel2017rainbow} further improves the sample efficiency by 
a combination of several extensions of DQN 
such as Double DQN~\cite{van2016deep}, Dueling networks~\cite{wang2015dueling}, 
prioritized experience replay~\cite{schaul2015prioritized}, 
multi-step learning~\cite{sutton2018reinforcement}.
The second category is the actor-critic approaches. Most of recent works~\cite{degris2012off,wang2016sample,gruslys2018reactor}
in this category leverage importance sampling by re-weighting the samples 
to correct the estimation bias. However, importance sampling usually involves  
a large variance and the truncated version could introduce bias to the gradient estimation.
Furthermore, one advantage of actor-critic methods is in the wall-clock times due 
to the distributed framework, firstly presented in~\cite{mnih2016asynchronous}, instead
of the sample-efficiency. As of the time of writing, the aggregate variant of DQN~\cite{hessel2017rainbow} is among the algorithms of most sample efficiency. 
In this work, we show that the ranking policy gradient can achieve better sample complexity than
the current state-of-the-art~\cite{hessel2017rainbow,dabney2018implicit,bellemare2017distributional,schaul2015prioritized,van2016deep}.

% imitation learning
\noindent\textit{Imitation Learning.}
In~\cite{hester2018deep}, hinge loss is combined with regular $Q$-learning loss 
as a pre-training step for learning from demonstration. The method 
used hinge loss as a regularization for imitating the expert behavior. Our analysis 
shows that the hinge loss can be directly used as a policy gradient method
and thus used as a regular 
reinforcement learning algorithm, which achieves higher sample-efficiency.
In behavior cloning~\cite{osa2018algorithmic}, hinge loss was used as a 
surrogate loss for imitating optimal trajectories. In this work, we show 
that RL can be cast to a supervised
learning problem, which naturally leads to sample-efficient off-policy learning,
without extensive parameter tuning~\cite{nachum2017bridging} or complicated adaptation~\cite{gu2016q,gruslys2018reactor,degris2012off}.
% imitation learning can be used to directly train the policy function 
% in a off-policy learning fashion.

\noindent\textit{RL as supervised learning}
% Numerous amount of works have studied the connection between RL and supervised learning.
Prior works on casting RL to supervised learning. 
Many of them worked on the maximum entropy objective~\cite{haarnoja2018soft,abdolmaleki2018maximum} 
while we focus on maximizing the long turn reward. Recently, preference based 
RL has arisen as an interesting topic in the field, 
where the reward signal is unknown while the trajectory preference is
assumed to be able to solicit from the experts~\cite{wirth2016model,furnkranz2012preference}. 
Also, there are works that cast RL into a EM framework, such as~\cite{dayan1997using,peters2007reinforcement}. In~\cite{dayan1997using}, the authors work on the simplified 
RL problem that the reward function is not associated with the state. In~\cite{peters2008reinforcement}, the authors transfer the maximizing of expected immediate reward into a EM algorithm. Different
from their setting, we consider maximizing the expected long term reward as a supervised 
learning problem and we explicitly describe the gap induced by this transformation.


% related work to ranking poilcy gradient. 
\noindent\textit{Ranking.}
RankNet~\cite{burges2005learning} provided a framework using gradient 
descent to learn from pairwise orders in the context of search ranking. 
ListNet~\cite{cao2007learning} proposed an approach to optimize 
the listwise relationship. The proposed ranking policy gradient methods
use the results from RankNet and ListNet to construct policy used for 
policy gradient.
% wclosely rely on those solid theoretical results and 


% related work to PAC learning and RL sample complexity
\noindent\textit{PAC Analysis in MDP.}
Piror sample complexity analysis~\cite{kakade2003sample,strehl2006pac,kearns2000approximate,strehl2009reinforcement,
krishnamurthy2016pac,jiang2017contextual,jiang2018open,zanette2019tighter} 
all established on the value function estimation. 
% Many of them work on the tabular-setting~\cite{kakade2003sample,strehl2006pac,zanette2019tighter},etc
% that is hard to scale to the MDP with large state space. To conduct analysis on large-scale MDP, 
% researchers propose rich observations~\cite{krishnamurthy2016pac,jiang2017contextual} that assuming
% the state space parti
In this work, we utilizes the probably approximately correct framework~\cite{valiant1984theory}
in a different way without relying on the value function, which directly leads
to a practical sample-efficient algorithm as we shown in the experiments. 

\noindent\textit{Cross-Entropy (CE) methods.}
Different from cross-entropy methods in reinforcement learning~\cite{de2005tutorial,szita2006learning,mannor2003cross},
our off-policy framework can utilize previous random trajectories repeatedly, which is more sample
efficient than CE since it is also a on-policy method. The randomly generated data can only be used 
for updating the policy once~\cite{szita2006learning,mannor2003cross}. \lkxcom{read~\cite{menache2005basis}}
% see alg 3.1 in mannor2003cross




